Multi-band Optical and Near-infrared Properties of Faint Submillimeter Galaxies with Serendipitous ALMA Detections

We present a catalog of 26 faint submillimeter galaxies (SMGs) in the XMM-LSS field identified by cross-matching serendipitously detected sources in archival ALMA Band 6 and 7 data with multi-band near-infrared (NIR) and optical data from the Spitzer Extragalactic Representative Volume Survey, the VISTA Deep Extragalactic Survey, the Canada-France-Hawaii Telescope Legacy Large Survey, and the Hyper Suprime-Cam Subaru Strategic Program. Of the 26 SMGs in our sample, 15 are identified here for the first time. The majority of the sources in our sample (16/26) have faint submm fluxes ($0.1\,{\rm mJy} < S_{\rm 1\,mm} < 1\,{\rm mJy}$). In addition to the 26 SMGs with multi-band optical and NIR detections, there are 60 highly-reliable ($>5\sigma$) ALMA sources with no counterpart in any other band down to an IRAC [4.5] $AB$ magnitude of $\approx 23.7$. To further characterize the 26 galaxies with both ALMA and optical/NIR counterparts, we provide 13-band forced photometry for the entire catalog using the Tractor and calculate photometric redshifts and rest-frame colors. The median redshift of our sample is $\langle z \rangle = 2.66$. We find that our sample galaxies have bluer colors compared to bright SMGs, and the UVJ color plot indicates that their colors are consistent with main sequence star-forming galaxies. Our results provide new insights into the nature of the faint population of SMGs, and also highlight opportunities for galaxy evolution studies based on archival ALMA data.

==> ContMaptab.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{longrotatetable}
\begin{deluxetable}{cccccccccc}
\tablecaption{Details of the archival observations and individual pointings \label{tab:tab1}}
\tabletypesize\scriptsize
\tablewidth{-2pt}
\tablehead{
\colhead{Index}           & \colhead{Map}      &
\colhead{RA}          & \colhead{Dec}  &
\colhead{Date of Observation}          & \colhead{Project ID}    &
\colhead{$\nu_{obs}$}  & \colhead{$\lambda_{obs}$ }  &
\colhead{Resolving Beam} & \colhead{RMS Noise} \\
& &(J2000) &(J2000) &($yyyy-mm-dd$) & &( GHz)& (mm)  & ($^{\prime\prime} \times ^{\prime\prime} $) & ($\mu$Jy beam$^{-1}$) }
\startdata
0 & CLM1 & 02h28m02.970s & -04d16m18.30s & 2014-06-16 & 2013.1.00815.S & 258 & 1.16 & 0.53 $\times$ 0.46 & 15.42 \\
1 & HiZELS-UDS-NBK-1147 & 02h17m37.000s & -05d09m12.00s & 2014-01-27 & 2012.1.00934.S & 222 & 1.35 & 1.64 $\times$ 0.7 & 58.27 \\
2 & HiZELS-UDS-NBK-1196 & 02h17m40.120s & -05d12m02.35s & 2014-01-27 & 2012.1.00934.S & 222 & 1.35 & 1.65 $\times$ 0.7 & 60.39 \\
3 & HiZELS-UDS-NBK-1348 & 02h17m51.470s & -05d10m36.40s & 2014-01-27 & 2012.1.00934.S & 222 & 1.35 & 1.65 $\times$ 0.7 & 59.21 \\
4 & HiZELS-UDS-NBK-8806 & 02h17m18.650s & -05d07m54.20s & 2014-01-27 & 2012.1.00934.S & 222 & 1.35 & 1.64 $\times$ 0.7 & 59.53 \\
5 & Himiko & 02h17m57.563s & -05d08m44.45s & 2012-07-15 & 2011.0.00115.S & 259 & 1.16 & 0.71 $\times$ 0.48 & 19.86 \\
6 & SXDF1100.013 & 02h16m46.210s & -05d03m47.83s & 2013-11-19 & 2012.1.00326.S & 265 & 1.13 & 0.57 $\times$ 0.38 & 81.4 \\
7 & SXDF1100.019 & 02h17m15.920s & -05d04m03.13s & 2013-11-19 & 2012.1.00326.S & 265 & 1.13 & 0.57 $\times$ 0.38 & 81.23 \\
8 & SXDF1100.027 & 02h17m20.550s & -05d08m42.36s & 2013-11-19 & 2012.1.00326.S & 265 & 1.13 & 0.57 $\times$ 0.38 & 80.98 \\
9 & SXDF1100.036 & 02h18m00.700s & -05d07m29.69s & 2013-11-19 & 2012.1.00326.S & 265 & 1.13 & 0.57 $\times$ 0.38 & 81.5 \\
10 & SXDF1100.039 & 02h18m30.590s & -05d01m16.09s & 2013-11-19 & 2012.1.00326.S & 265 & 1.13 & 0.57 $\times$ 0.38 & 79.86 \\
11 & SXDF1100.045 & 02h18m15.350s & -04d54m03.36s & 2013-11-19 & 2012.1.00326.S & 265 & 1.13 & 0.57 $\times$ 0.38 & 79.46 \\
12 & SXDF1100.049 & 02h17m33.310s & -04d57m02.02s & 2013-11-19 & 2012.1.00326.S & 265 & 1.13 & 0.57 $\times$ 0.38 & 81.66 \\
13 & SXDF1100.053 & 02h16m48.170s & -04d58m56.66s & 2013-11-19 & 2012.1.00326.S & 265 & 1.13 & 0.57 $\times$ 0.38 & 82.26 \\
14 & SXDF1100.060 & 02h17m37.700s & -05d08m23.17s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.68 $\times$ 0.48 & 137.39 \\
15 & SXDF1100.063 & 02h17m35.990s & -04d52m18.15s & 2013-11-19 & 2012.1.00326.S & 265 & 1.13 & 0.57 $\times$ 0.38 & 80.8 \\
16 & SXDF1100.073 & 02h18m10.270s & -05d11m26.18s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.68 $\times$ 0.48 & 141.14 \\
17 & SXDF1100.082 & 02h17m58.290s & -04d59m11.16s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.69 $\times$ 0.48 & 141.18 \\
18 & SXDF1100.083 & 02h17m11.830s & -05d03m59.71s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.69 $\times$ 0.48 & 143.26 \\
19 & SXDF1100.090 & 02h17m23.660s & -04d57m24.06s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.69 $\times$ 0.48 & 139.67 \\
20 & SXDF1100.101 & 02h18m35.580s & -05d10m02.67s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.69 $\times$ 0.48 & 139.46 \\
21 & SXDF1100.104 & 02h18m04.930s & -05d08m19.32s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.68 $\times$ 0.48 & 141.65 \\
22 & SXDF1100.109 & 02h18m23.720s & -05d08m05.49s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.69 $\times$ 0.48 & 140.09 \\
23 & SXDF1100.110 & 02h17m44.200s & -05d04m08.78s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.69 $\times$ 0.48 & 141.69 \\
24 & SXDF1100.123 & 02h18m11.930s & -05d14m20.94s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.69 $\times$ 0.48 & 138.85 \\
25 & SXDF1100.127 & 02h17m33.080s & -04d48m51.89s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.64 $\times$ 0.46 & 65.92 \\
26 & SXDF1100.154 & 02h18m14.490s & -04d56m12.80s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.64 $\times$ 0.46 & 63.9 \\
27 & SXDF1100.174 & 02h18m16.350s & -05d15m28.80s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.64 $\times$ 0.46 & 64.95 \\
28 & SXDF1100.179 & 02h18m43.870s & -04d57m33.62s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.64 $\times$ 0.46 & 64.43 \\
29 & SXDF1100.230 & 02h17m58.610s & -04d45m49.13s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.64 $\times$ 0.46 & 64.6 \\
30 & SXDF1100.231 & 02h17m59.910s & -04d46m50.05s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.64 $\times$ 0.46 & 65.54 \\
31 & SXDF1100.233 & 02h18m53.030s & -04d58m14.74s & 2013-11-19 & 2012.1.00326.S & 265 & 1.13 & 0.57 $\times$ 0.38 & 81.82 \\
32 & SXDF1100.250 & 02h17m52.690s & -05d20m31.72s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.64 $\times$ 0.46 & 64.78 \\
33 & SXDF1100.253 & 02h18m26.970s & -05d14m38.61s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.64 $\times$ 0.46 & 64.45 \\
34 & SXDF1100.276 & 02h18m33.930s & -04d54m23.85s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.64 $\times$ 0.46 & 66.35 \\
35 & SXDF1100.277 & 02h17m24.090s & -05d20m21.94s & 2013-11-30 & 2012.1.00326.S & 265 & 1.13 & 0.64 $\times$ 0.46 & 63.16 \\
36 & SXDF.220GHZ & 02h18m56.536s & -05d19m58.92s & 2014-05-03 & 2012.1.00374.S & 224 & 1.33 & 0.82 $\times$ 0.62 & 12.56 \\
37 & SXDF-NB1 & 02h18m56.536s & -05d19m58.92s & 2015-12-27 & 2013.A.00021.S & 224 & 1.33 & 1.94 $\times$ 1.07 & 15.1 \\
38 & SXDS1\_13015 & 02h17m13.617s & -05d09m39.82s & 2012-08-15 & 2011.0.00648.S & 243 & 1.23 & 0.8 $\times$ 0.58 & 100.87 \\
39 & SXDS1\_1723 & 02h17m32.701s & -05d13m16.47s & 2012-08-26 & 2011.0.00648.S & 240 & 1.25 & 1.11 $\times$ 0.59 & 111.28 \\
40 & SXDS1\_33244 & 02h16m47.397s & -05d03m28.09s & 2012-08-26 & 2011.0.00648.S & 240 & 1.25 & 0.95 $\times$ 0.59 & 77.72 \\
41 & SXDS1\_35572 & 02h17m34.652s & -05d02m38.97s & 2012-08-11 & 2011.0.00648.S & 236 & 1.27 & 0.78 $\times$ 0.58 & 46.17 \\
42 & SXDS1\_59863 & 02h17m45.877s & -04d54m37.60s & 2012-08-15 & 2011.0.00648.S & 243 & 1.23 & 0.81 $\times$ 0.58 & 95.02 \\
43 & SXDS1\_59914 & 02h17m12.977s & -04d54m40.40s & 2012-08-26 & 2011.0.00648.S & 240 & 1.25 & 1.04 $\times$ 0.59 & 109.0 \\
44 & SXDS1\_67002 & 02h19m02.654s & -04d49m55.83s & 2012-08-15 & 2011.0.00648.S & 243 & 1.23 & 0.83 $\times$ 0.57 & 97.8 \\
45 & SXDS1\_68849 & 02h17m00.276s & -04d48m14.53s & 2012-08-26 & 2011.0.00648.S & 240 & 1.25 & 0.85 $\times$ 0.6 & 96.21 \\
46 & SXDS1\_79518 & 02h18m59.059s & -04d51m24.91s & 2012-08-26 & 2011.0.00648.S & 240 & 1.25 & 0.9 $\times$ 0.6 & 99.08 \\
47 & SXDS1 & 02h17m05.789s & -04d51m25.68s & 2012-08-09 & 2011.0.00648.S & 231 & 1.3 & 0.8 $\times$ 0.67 & 64.28 \\
48 & SXDS2\_13316 & 02h17m39.035s & -04d44m41.75s & 2012-08-15 & 2011.0.00648.S & 243 & 1.23 & 0.81 $\times$ 0.57 & 92.28 \\
49 & SXDS2\_22198 & 02h17m53.416s & -04d42m53.42s & 2012-08-11 & 2011.0.00648.S & 236 & 1.27 & 0.81 $\times$ 0.58 & 44.84 \\
50 & SXDS2 & 02h17m24.356s & -05d00m44.85s & 2012-08-09 & 2011.0.00648.S & 231 & 1.3 & 0.8 $\times$ 0.66 & 63.38 \\
51 & SXDS3\_101746 & 02h18m04.178s & -05d19m38.28s & 2012-08-26 & 2011.0.00648.S & 240 & 1.25 & 0.93 $\times$ 0.6 & 99.25 \\
52 & SXDS3\_103139 & 02h16m57.652s & -05d14m34.86s & 2012-08-11 & 2011.0.00648.S & 236 & 1.27 & 0.77 $\times$ 0.58 & 46.08 \\
53 & SXDS3\_110465 & 02h18m20.953s & -05d19m07.71s & 2012-08-26 & 2011.0.00648.S & 240 & 1.25 & 0.99 $\times$ 0.6 & 99.74 \\
54 & SXDS3 & 02h17m13.683s & -05d04m07.66s & 2012-08-09 & 2011.0.00648.S & 231 & 1.3 & 0.81 $\times$ 0.66 & 60.34 \\
55 & SXDS5\_19723 & 02h16m24.372s & -05d09m18.05s & 2012-08-11 & 2011.0.00648.S & 236 & 1.27 & 0.77 $\times$ 0.58 & 45.41 \\
56 & SXDS5\_28019 & 02h16m08.532s & -05d06m15.61s & 2012-08-11 & 2011.0.00648.S & 236 & 1.27 & 0.78 $\times$ 0.58 & 46.36 \\
57 & SXDS5\_9364 & 02h16m33.807s & -05d13m44.68s & 2012-08-15 & 2011.0.00648.S & 243 & 1.23 & 0.81 $\times$ 0.57 & 97.7 \\
58 & UDS16 & 02h17m25.474s & -05d11m08.25s & 2016-03-31 & 2015.1.01105.S & 241 & 1.24 & 0.96 $\times$ 0.8 & 21.5 \\
59 & WMH5 & 02h26m27.030s & -04d52m38.30s & 2014-06-16 & 2013.1.00815.S & 262 & 1.14 & 0.5 $\times$ 0.48 & 18.05 \\
60 & XMMF10 & 02h16m31.850s & -05d53m22.20s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.41 & 220.03 \\
61 & XMMF11 & 02h21m35.220s & -06d26m16.97s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.41 & 261.51 \\
62 & XMMF12 & 02h22m50.830s & -03d24m13.81s & 2012-06-17 & 2011.0.00539.S & 342 & 0.87 & 0.49 $\times$ 0.41 & 212.05 \\
63 & XMMF13 & 02h18m41.550s & -03d50m01.90s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.41 & 227.81 \\
64 & XMMF14 & 02h20m29.140s & -06d48m45.89s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.41 & 236.57 \\
65 & XMMF15 & 02h22m05.540s & -07d07m27.20s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.41 & 212.96 \\
66 & XMMF16 & 02h19m42.910s & -05d24m32.54s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.41 & 224.83 \\
67 & XMMF17 & 02h19m18.400s & -03d10m51.30s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.42 & 259.53 \\
68 & XMMF18 & 02h29m44.790s & -03d41m10.17s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.52 $\times$ 0.41 & 300.12 \\
69 & XMMF19 & 02h20m21.610s & -01d53m29.12s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.52 $\times$ 0.42 & 277.51 \\
70 & XMMF25 & 02h22m50.830s & -03d24m13.80s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.57 $\times$ 0.51 & 500.26 \\
71 & XMMF4 & 02h20m16.689s & -06d01m44.38s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.41 & 262.64 \\
72 & XMMF5 & 02h22m01.576s & -03d33m40.60s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.52 $\times$ 0.41 & 233.23 \\
73 & XMMF6 & 02h25m48.210s & -04d17m51.10s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.41 & 254.89 \\
74 & XMMF7 & 02h18m53.100s & -06d33m23.70s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.41 & 219.54 \\
75 & XMMF8 & 02h30m05.980s & -03d41m52.70s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.52 $\times$ 0.41 & 254.45 \\
76 & XMMF9 & 02h18m30.740s & -05d31m30.80s & 2012-06-17 & 2011.0.00539.S & 343 & 0.87 & 0.51 $\times$ 0.41 & 357.21 \\
\enddata
\end{deluxetable}
\end{longrotatetable}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> oldtext.tex <==
\textbf{oldtext}

\textbf{Properties of bright SMGs and status of their surveys}

The most luminous DSFGs have extreme environments with SFRS going upto thousands of solar masses per year. Some of them have AGN and having intense starburst in the compact central region. These galaxies will soon reveal the central AGN becoming luminous quasars. Up until now, single dish observations using SCUBA as well as space telescopes like Spitzer and Herschel have revealed millions of SMGs with a median redshift of 2.2 (Check it again in the Blain 2003 review). Poor spatial resolution and confusion limit ($\sim$2mJy at 850 $\mu$m ) are main challenges for the deep high resolution surveys. .
Also, these populations did not contribute significantly to the EBL at IR (Need references). Therefore there exists fainter population which is very important. Gravitational lensing studies have allowed us to go below the detection limit to study the fainter population (Hsu and Other References). This method has very large uncertainties due to inaccuracy of lensing models and sample is limited as you need a cluster in the foreground. 
\subsection{ALMA archival data}

We have mined through ALMA archive to search for any observations within the XMM field. The observations that became available to the public by July 2017 and satisfied following criteria were selected. 
%We have used archival data in band 6 or 7 that was available to public by July 2017. 
The criteria were 1) The observations should be in band 6 or 7. 2) The time integration should be greater than 150s 3) The angular resolution should be greater than 0.4$^"$. As we are dealing with fainter population, the rms noise levels should be low enough to have strong detection. The reason behind third criterion is source cross-matching.  We need comparable resolution to perform the cross matching with NIR observations from SERVS. Our search covered 69 maps from 9 different projects. Table \ref{tab:tab1} summarizes the list of all the projects that we used from the archive. The angular resolutions in the archival data ranged from 0.53" to 1.46". All of the observations are taken in the band 6. The typical RMS noise levels range from 15$\mu$Jy to 200 $\mu Jy$. Therefore, the search depth is not uniform throughout our search. 


\subsection{Optical/NIR observations}

The Sources selected from ALMA observations were cross matched to find counterparts in the \textcolor{yellow}{12} bands.The data include 3.6 and 4.5 micron post-cryogenic observations taken using IRAC on Spitzer satellite. Complimentary ground-based observations are available for all five SERVS fields. The NIR photometry include Z, Y, J, H, and $K_{s}$ bands from VISTA Deep Extragalactic Survey (VIDEO;Jarvis et al. 2013). A part of the XMM field is covered by Canada-France-Hawaii Telescope Legacy Survey Wide Field 1 (CFHTLS-W1). The optical observations from CFHTLS-W1 include $u^{'}$, $g^{'}$, $r^{'}$, $i^{'}$, and $z^{'}$ bands. So, in total 12 optical/NIR bands are included to find counterparts for submm sources. The final catalog was also cross-matched with Herschel Multitiered Extragalactic Survey; HerMES (Oliver et al. 2012).


\subsection{Data Reduction} 

The entire data calibration and imaging was done in the software package Common Astronomy Software Application (CASA). We have used same CASA version as the one used in the calibration pipeline. The data was reduced in a standard manner using calibration scripts provided by the ALMA observatory. All of the data covers cycles from 0 to 3. The calibration script performs initial flagging, bandpass calibration and gain calibration. The calibrated dataset were imaged using task CLEAN in the CASA. Unless required the imaging parameters were taken from the provided scripts. Some of the observations had image artifacts such as stripe patterns. We performed additional flagging, re-calibration  and reimaging for such cases. For the cycle 0, the calibrated measurement set was provided. Also, the script CASA version was unavailable. So, version 4.5.2 was used instead to image the measurement set.  

When imaging using script parameters, we have found that the threshold has not been set non-zero value. This would result in cleaning the noise peaks as a real source. As a result, the noise was lower but the noise will be selected as a real source increasing spurious sources. Therefore, we applied a clean threshold of 2$\sigma$ and provided a clean mask for bright sources. Briggs weighting with robust parameter of 0.5 was used in most cases. In case, there was a bright source in the target field, phase self calibration was performed to improve sensitivity of the image.
